Proper Jordan schemes exist. First examples, computer search, patterns of reasoning. An essay

A special class of Jordan algebras over a field $F$ of characteristic zero is considered. Such an algebra consists of an $r$-dimensional subspace of the vector space of all square matrices of a fixed order $n$ over $F$. It contains the identity matrix, the all-one matrix; it is closed with respect to \correction{matrix transposition}, Schur-Hadamard (entrywise) multiplication and the Jordan product $A*B=\frac 12 (AB+BA)$, where $AB$ is the usual matrix product. The suggested axiomatics (with some natural additional requirements) implies an equivalent reformulation in terms of symmetric binary relations on a vertex set of cardinality $n$. The appearing graph-theoretical structure is called a Jordan scheme of order $n$ and rank $r$. A significant source of Jordan schemes stems from the symmetrization of association schemes. Each such structure is called a non-proper Jordan scheme. The question about the existence of proper Jordan schemes was posed a few times by Peter J. Cameron. In the current text an affirmative answer to this question is given. The first small examples presented here have orders $n=15,24,40$. Infinite classes of proper Jordan schemes of rank 5 and larger are introduced. A prolific construction for schemes of rank 5 and order $n=\binom{3^d+1}{2}$, $d\in {\mathbb N}$, is outlined. The text is written in the style of an essay. The long exposition relies on initial computer experiments, a large amount of diagrams, and finally is supported by a number of patterns of general theoretical reasonings. The essay contains also a historical survey and an extensive bibliography.

==> figure.9.vertices.tex <==

  \node
  (14) at (0,4) {14};
  \node
  (13) at (0,2) {13};
  \begin{scope}[rotate around={36:(0,0)}]
    \node
    (3) at (0,6) {3};
  \end{scope}
  
  \begin{scope}[rotate around={72:(0,0)}]
    \node
    (9) at (0,4) {9};
    \node
    (8) at (0,2) {8};
    \begin{scope}[rotate around={36:(0,0)}]
      \node
      (4) at (0,6) {4};
    \end{scope}
  \end{scope}

  \begin{scope}[rotate around={144:(0,0)}]
    \node
    (11) at (0,4) {11};
    \node
    (1) at (0,2) {1};
    \begin{scope}[rotate around={36:(0,0)}]
      \node
      (12) at (0,6) {12};
    \end{scope}
  \end{scope}

  \begin{scope}[rotate around={216:(0,0)}]
    \node
    (5) at (0,4) {5};
    \node
    (7) at (0,2) {7};
    \begin{scope}[rotate around={36:(0,0)}]
      \node
      (0) at (0,6) {0};
    \end{scope}
  \end{scope}

  \begin{scope}[rotate around={288:(0,0)}]
    \node
    (6) at (0,4) {6};
    \node
    (10) at (0,2) {10};
    \begin{scope}[rotate around={36:(0,0)}]
      \node
      (2) at (0,6) {2};
    \end{scope}
  \end{scope}


==> klein.vertices.tex <==

  \node (a1) at (0,2) {26};
  \node (a2) at (0,4.5) {35};
  \node (a3) at (0,-6) {01}; 
  \begin{scope}[rotate around={180+25.7:(0,0)}]
  \node (b1) at (0,2) {36};
  \node (b2) at (0,4.5) {02};
  \node (b3) at (0,-6) {45}; 
  \end{scope}
  \begin{scope}[rotate around={51.4:(0,0)}]
  \node (c1) at (0,2) {03};
  \node (c2) at (0,4.5) {46};
  \node (c3) at (0,-6) {12}; 
  \end{scope}
  \begin{scope}[rotate around={180+77.1:(0,0)}]
  \node (d1) at (0,2) {04};
  \node (d2) at (0,4.5) {13};
  \node (d3) at (0,-6) {56} ;
  \end{scope}
  \begin{scope}[rotate around={102.8:(0,0)}]
  \node (e1) at (0,2) {14};
  \node (e2) at (0,4.5) {05};
  \node (e3) at (0,-6) {23} ;
  \end{scope}
  \begin{scope}[rotate around={180+128.5:(0,0)}]
  \node (f1) at (0,2) {15};
  \node (f2) at (0,4.5) {24};
  \node (f3) at (0,-6) {06} ;
  \end{scope}
  \begin{scope}[rotate around={154.2:(0,0)}]
  \node (g1) at (0,2) {25};
  \node (g2) at (0,4.5) {16};
  \node (g3) at (0,-6) {34} ;
  \end{scope}

